Rapid acceleration of electrons in the magnetosphere by fast-mode MHD waves

During major megnetic storms, enhanced flux of relativistic electrons in the inner magnetosphere have been observed to correleated with ULF waves. The enhancements can take place over a period of several hours. In order to account for such a rapid generation of relativistic electrons, we examine the mechanism of transit-time acceleration of electrons by low-frequency fast-mode MHD waves, here the assumed form of ULF waves. Calcaulations of the acceleration timescales in the model show that fast-mode waves in the Pc4 to Pc5 frequency range, with typically observed wave amplitudes 10--20 nT, can accelerate the seed electrons to energies of order MeV in a period of a few hours.

==> update.tex <==
%auto-ignore
%%  update.tex -- August 6, 1996 version
%
%%  revisions by Amy Hendrickson, TeXnology Inc.

%   You may not need this file unless you have 
%   a very old version of LaTeX 2.09.
%
%   This file keeps old versions of LaTeX 2.09 
%   from becoming confused with \reset@font and 
%   thus crashing at every undefined label or 
%   citation.  
%
%   If you do need to include this file, 
%   type \input{update.tex} in front of your 
%   \begin{document} command in your *.tex
%   file and then continue as you would ordinarily.

\makeatletter
\let\reset@font\empty
\makeatother

